ERRANT: Realistic Emulation of Radio Access Networks

Mobile networks have become ubiquitous, but running experiments on them is expensive and hard, given their complexity and diversity. Emulation can be the solution, and, with ERRANT, we offer a realistic emulator of mobile networks based on a large measurement campaign on European Mobile Network Operators. It improves the current situation, where tools and emulators only implement pre-defined profiles, with built-in parameters, which are not supported with real measurements.

==> makefile <==
DOC=main

all:
	pdflatex $(DOC)
	bibtex   $(DOC)
	pdflatex $(DOC)
	pdflatex $(DOC)

clean:
	find . -name '*~' -exec rm -f {} \;
	find . -name '*.aux' -exec rm -f {} \;
	rm -f texput.log $(DOC).log $(DOC).ps $(DOC).toc $(DOC).lo* $(DOC).bbl $(DOC).blg $(DOC).dvi $(DOC).out $(DOC).synctex.gz diff.bbl diff.blg

zip: ${sources} ${pdffiles}
	rm -f $(DOC).zip && zip -r $(DOC).zip *.tex *.bib *.bbl *.cls figures Makefile makefile

diff:
		latexdiff -c submission_version/latexdiff_conf.txt \
							--preamble=submission_version/latexdiff_preamble_old.tex \
		          --exclude-textcmd="subsection" \
	            --flatten submission_version/main.tex main.tex > diff.tex
		#pdflatex diff
		#bibtex diff
		pdflatex diff
		pdflatex diff

